Taking Care of The Discretization Problem: A Comprehensive Study of the Discretization Problem and A Black-Box Adversarial Attack in Discrete Integer Domain

Numerous methods for crafting adversarial examples were proposed recently with high success rate. Since most existing machine learning based classifiers normalize images into some continuous, real vector, domain firstly, attacks often craft adversarial examples in such domain. However, "adversarial" examples may become benign after denormalizing them back into the discrete integer domain, known as the discretization problem. This problem was mentioned in some work, but has received relatively little attention. In this work, we first conduct a comprehensive study of existing methods and tools for crafting. We theoretically analyze 34 representative methods and empirically study 20 representative open source tools for crafting adversarial images. Our study reveals that the discretization problem is far more serious than originally thought. This suggests that the discretization problem should be taken into account seriously when crafting adversarial examples and measuring attack success rate. As a first step towards addressing this problem in black-box scenario, we propose a black-box method which reduces the adversarial example searching problem to a derivative-free optimization problem. Our method is able to craft adversarial images by derivative-free search in the discrete integer domain. Experimental results show that our method is comparable to recent white-box methods (e.g., FGSM, BIM and C\&W) and achieves significantly higher success rate in terms of adversarial examples in the discrete integer domain than recent black-box methods (e.g., ZOO, NES-PGD and Bandits). Moreover, our method is able to handle models that is non-differentiable and successfully break the winner of NIPS 2017 competition on defense with 95\% success rate. Our results suggest that discrete optimization algorithms open up a promising area of research into effective black-box attacks.

==> experiments-newdata.tex <==
\section{Implementation and Evaluation}
\label{sec:expr}
\subsection{Implementation}
We implement our method into a black-box style adversary example generation tool \tool.
%As described before, our method is derivative-free optimization based.
We also implement a derivative-free optimization engine in \tool based on RACOS~\cite{yu2016derivative},
for which we manage to engineer to significantly improve its efficiency
and scalability with lots of domain-specific optimizations.
Due to the space limitation,  details of the optimizations are omitted here. % is dismissed here.

%We make a brand new re-implementation, following the code structure of RACOS,
%with sets of domain-related optimizations and other engineering-aspect optimizations for performance increasing. Due to the space limitation,  the detail of the optimization done in the implementation is dismissed here.

In order to process pre-trained networks (e.g., InceptionV3), we also integrate TensorFlow (V1.8.0)~\cite{abadi2016tensorflow} and Keras (V2.1.6)~\cite{keras19} DL frameworks
in our tool for image prediction.
Besides integer adversarial example generation for well-known image classification models,
our tool can be easily expanded to adapt non-image classification models as well,
by customizing the interfaces in our tool, e.g., the dissatisfaction-degree function.



%Actually, the models that can be handled by our implementation are not necessarily focusing on image classification. If the user has customized the corresponding evaluation functions, and optimization problems, which is also very easy to conduct by taking advantage of the interface given in our implementation, our implementation can handle the adversary example generation of certain model easily as we conduct a black-box style searching and do not require the inner information of the model.

%Our tool provides the following functionalities:
%\begin{itemize}
%\item Provide interfaces of classification model and input, and generate the corresponding adversarial examples automatically.
%\item Provide parameter strategy. ABC provides multiple parameters strategies to deal with different data sets and attack patterns.
%\item Provide interface to customize evaluation function. ABC provides multiple evaluation functions for different optimization problems and provides interface for custom problems.
%\end{itemize}
%Based on the above, our tools are easy to reproduce and expand. Users can use the neural network in Keras's applications by default or submit their own classification model. Similarly, users also can customize optimization problems and dissatisfaction-degree functions or use the default configuration.

%Regarding the RACOS source code, we have made some engineering optimizations based on the adversarial examples generation problem, which greatly reduces the time cost without reducing the effect. In detail:
%\begin{itemize}
%\item Minimize the use of the for-loop because that Python executes very slowly on the for-loop. We use the operation in numpy to simulate the function in source code.
%\item Cancel the steps to avoid resampling when the same solutions are sampled. For the concrete problem, the probability of getting the same solutions is small enough to be ignored because that the sampling space is too large. Even if it happens, just the resource of sampling once is waste.
%\item There are other tricks used to increase efficiency.
%\end{itemize}

%All in all, we implement an adversarial example generator ABC, which is efficient and convenient to extend.
\subsection{Dataset \& Setting}
We use two datasets MNIST and ImageNet in this section.

\medskip
\noindent
\textbf{MNIST.} MNIST~\cite{MNIST98} is a dataset of handwritten digits and contains $28\times28\times1$ pixel images with $10$ classes (0-9).
%MNIST includes $60000$ images for training and $10000$ images for validation.
We choose the first 200 images out of $10000$ validation images of MNIST as our subjects.
We evaluate MNIST images using LeNet-1, a DNN classifier from the LeNet family~\cite{LBBH98}.

\medskip
\noindent
\textbf{ImageNet.} ImageNet~\cite{DDSLL009} is a large image dataset.
The size of images in ImageNet is around $299\times299\times3$ or $224\times224\times3$ pixels.
ImageNet contains over $10000000$ images with $1000$ classes.
We choose 100 images which can be correctly classified by four classifiers of Keras (i.e., ResNet50, IncepetionV3, VGG16 and VGG19).
We use two well-known pre-trained DNN, ResNet50~\cite{HZRS16} and InceptionV3~\cite{SVISW16} as the target DNN classifiers in our experiments.

%Among all these three target networks, we can basically rank the difficulties of attacking these models as InceptionV3 > ResNet50 > LeNet-1.

%We conduct both untargeted attack and targeted attack in the experiments. All experiments are run on a Linux PC running UBUNTU 16.04 LTS with Intel Xeon(R) W-2123 CPU, TITAN Xp COLLECTORS GPU and 64G RAM. Table~\ref{tab:set} lists the other settings used.


%For MNIST, our target DNN network is
% ut of the total $10000$ images in the validation set, we use the beginning 200 images as the image set for the experiment.\\
%\textbf{ImageNet.} Compared with MNIST, ImageNet~\cite{DDSLL009} is a considerably large image dataset.  The size of images in ImageNet is around $299\times299\times3$ or $224\times224\times3$ pixels, which is much more larger than MNIST. ImageNet contains over $10000000$ images with $1000$ classes. We use 100 images that all can be correctly classified by all the Keras tools as described in Sect.3.2.1 for experiments. We use two well-known pre-trained DNN, ResNet50~\cite{HZRS16} and InceptionV3~\cite{SVISW16} as the target DNN in the experiment.

%Among all these three target networks, we can basically rank the difficulties of attacking these models as InceptionV3 > ResNet50 > LeNet-1.

%As reported in~\cite{chollet2015keras}, the accuracy of nceptionV3 is larger than ResNet50. Compared with the network on ImageNet with LeNet-1, the

%and randomly select 100 images for attack.

%The image set selection is more tricky compared with MNIST. We download the subset of ImageNet{\footnote{http://jaina.cs.ucdavis.edu/datasets/adv/imagenet/img.tar.gz}}, which was used in the evaluation of ZOO~\cite{CZSYH17}. Then we use 100 images that all can be correctly classified by all the keras tools\footnote{\url{https://keras.io.}}.
%
%
%This set contains $50$ images for each of the $1000$ categories. At first, we select $100$ categories out of the $1000$ categories randomly. Then, to increase the difficulty of adversary attack, for these $50$ images, we send them to several different DNN models, including ResNet50, IncepetionV3, VGG16 and VGG19, for classification. The first image which achieves consensus result from all the models will be selected into our data set for experiment. So, at last we get $100$ images from ImageNet for the experiment.

We conduct both untargeted attack and targeted attack in the experiments,
on a Linux PC running UBUNTU 16.04 LTS with Intel Xeon(R) W-2123 CPU, TITAN Xp COLLECTORS GPU and 64G RAM. Table~\ref{tab:set} lists the other settings used.


\begin{table}
\small
\begin{tabular}{p{1.6cm}|p{6cm}}
  \hline
  \textbf{Parameter} & \textbf{Setting} \\ \hline

$\mathds{L}_\infty$ distance & $\epsilon=64$ for MNIST and $\epsilon=10$ for ImageNet. \\ \hline
  Target  & For MNIST, the class with $4$-th highest probability. \\
  class   & For ImageNet,the class with $11$-th highest probability. \\ \hline
  Sample & $s=5$ for untargeted attack. \\
  size $s$ & $s=10$ for targeted attack. \\\hline
  Ranking Threshold&  {\color{red} $k=3$} in all the experiments. \\\hline
  Coordinate Threshold & The number of coordinates that can be modified in the perturbation during each iteration.   $2$ pixels for MNIST and {\color{red} $200$} pixels for ImageNet.\\\hline
  Iteration  & $T=10000$ in all the experiments.\\
     Threshold & \\ \hline
  Timeout  & 3 minutes for MNIST  . \\
   Threshold & 30 minutes for ImageNet. \\\hline

\end{tabular}
\caption{Experiment Setting.}
\label{tab:set}
\end{table}


Besides the SR, TSR, and GAP metrics defined in Section~\ref{sec:DPprobleminWild},
we use ATC to denote the average time cost per real adversarial example in second for other tools,
and the average time cost per integer adversarial example in second for our tool.

%\textbf{MP.} The maximum value that each coordinate in the perturbation can be modified is 64 for MNIST and 10 for ImageNet. In another word, we are using the ${\bf L}_\infty$ distance in the experiment.\\
%\textbf{Target Label.} For targeted attack, we chose the label with the $4$th high probability as the target label for each image in MNIST. While for ImageNet, the target label is the $11$th in the original classification.\\
%\textbf{Time Limitation.} As we can see from the above setting, the problem on ImageNet is much difficult than the ones on MNIST, we set the time limitation as 3 minutes for MNIST and 30 minutes for ImageNet.




%We use the following metrics for the evaluation:\\
%\textbf{Success Rate(SR).} We use $NUM_{method}$ to denote the number of images considered successful attacked by the corresponding methods and $NUM_{all}$ to represent the size of input set. We use $NUM_{method}/NUM_{all}$ to represent success rate, or in other words, the traditional success rate.\\
%\textbf{True Success Rate(ASR).} As presented in Section 3, there is a gap between the success attack on the vector level and the discrete image level. Therefore, we map back the  $NUM_{method}$ perturbations to the real discrete image and ask the corresponding model to classify them again.
%We denote the number of elements in the subset which is attack the discrete image successfully as  $NUM_{real}$, and define the actual success rate as $NUM_{real}/NUM_{all}$.\\
%%\textbf{True Success Rate(TSR).} Based on the definitions of SR and ASR, we define the true success rate (TSR) as $SR\times ASR$, ie $NUM_{real}/NUM_{all}$\\
%\textbf{Average Time Cost(ATC).} ATC makes an investigation of the average time usage, in the unit of seconds, of the successful attacks, to measure the efficiency of the corresponding attacking methods.
%black-box

%It is the exist of time out so that the time cost of fail cases does not make sense. Thus for ATC we only consider the time cost of success cases.



\subsection{Comparison with White-Box Methods}
%Our method is fast to generate adversarial examples with high success, thus we can compare with white-box method.
Although our method is black-box based,
we compare the performance of our tool with two well-known gradient-based white-box tools: FGSM~\cite{GSS15}, BIM~\cite{KGB17}, and C\&W~\cite{CW17b}.
The $\mathds{L}_\infty$ distances are transformed into their ${\bf L}_\infty$ distances accordingly.

The results are shown in Table~\ref{tab:wu} and Table~\ref{tab:wt} for
untargeted and targeted attacks, respectively.
In terms of traditional attack success rate (SR),
\tool is comparable with  FGSM~\cite{GSS15}, BIM~\cite{KGB17} and C\&W~\cite{CW17b}.
In terms of attack true success rate (TSR), our tool \tool outperforms FGSM~\cite{GSS15} and C\&W~\cite{CW17b}. in most cases.
It is not surprising that our black-box tool \tool requires more time than other white-box methods.



Similar to the results given in Table~\ref{tab:TheExpofDP},
we can see that  C\&W has a huge gap of targeted attacks on InceptionV3 in ${\bf L}_\infty$ setting,
as its TSR is only $24\%$ compared with $100\%$ SR.
Thus, although C\&W outperforms \tool in terms of SR,
\tool outperforms C\&W  in most cases in terms of TSR. Different from C\&W, the step size of BIM can be set as integer. Under such setting, BIM does not have issue in discretization problem and performs very well in almost all the cases. Nevertheless, our tool \tool is compatible with BIM in terms of TSR in almost all the cases.

%
%
%As reported in Table~\ref{tab:TheExpofDP}, the current vector attack may face the issue of the discretization problem. Consistent with the report given in Table~\ref{tab:TheExpofDP}, we can see that on the aspect of TSR, C\&W has a huge gap in the ${\bf L}_\infty$ setting, that the TSR of C\&W on InceptionV3 in the targeted mode is only $24\%$. As the search space of our method is an integer domain, our method does not have such an issue. Thus, although the value of SR of C\&W is higher than our tool in several cases, the final TSR of our methods outperform C\&W in most of the cases.
%
%Another white-box method FGSM only needs one step to generate the adversarial examples, therefore it seldom shows the gap between TSR and SR in the experiment. However, FGSM has nearly no ability to handle targeted attack. Meanwhile, it is not surprising to see the time usage of our methods is higher than white-box methods, as they are using gradient information to help with the convergence to the correct solution.


%All in all, our tool is not worse in traditional metric but better in the new metric proposed by us.




%so that they are fast with high success rate. We compare them with our tool in MNIST and ImageNet.
%\begin{table}[htbp]
%  \centering
%\caption{Comparison with white-box methods with untarget attack mode}
%\label{tab:wu}
%\resizebox{85mm}{!}{
%\begin{tabular}{|c|c|c|c|c|c|c|}\hline
%Dataset&DNN&Method&SR&ASR&TSR&ATC\\
%\hline
%\multirow{3}*{MNIST}&\multirow{3}*{LeNet}&C\&W&100\%&85\%&85\%&14.3\\
%~&~&FGSM&96.7\%&100\%&96.7\%&0\\
%~&~&\tool&100\%&100\%&100\%&1.2\\
%\hline
%\multirow{3}*{ImageNet}&\multirow{3}*{ResNet50}&C\&W&99\%&100\%&99\%&8.56\\
%~&~&FGSM&94.8\%&100\%&94.8\%&0.08\\
%~&~&\tool&90\%&100\%&90\%&65\\
%\hline
%\multirow{3}*{ImageNet}&\multirow{3}*{InceptionV3}&C\&W&100\%&68\%&68\%&5.88\\
%~&~&FGSM&76\%&100\%&76\%&0.15\\
%~&~&\tool&{93\%}&100\%&{93\%}&{106.8}\\
%\hline
%\end{tabular}}
%\end{table}

\begin{table}[t]
  \centering

\caption{Results of white-box untargeted attacks.}
\label{tab:wu}
\resizebox{75mm}{!}{
\begin{tabular}{|c|c|c|c|c|c|c|}\hline
{\bf Dataset}&{\bf DNN}&{\bf Method}&{\bf SR}&{\bf TSR}&{\bf GAP}&{\bf ATC}\\
\hline
\multirow{4}*{MNIST}&\multirow{4}*{LeNet-1}&FGSM&96.7\%&96.7\%&0\%&0\\
~&~&BIM&100\%&{\bf 100\%}&0\%&0.01\\
~&~&C\&W&100\%&85\%&15\%&14.3\\
~&~&\tool&100\%&{\bf 100\%}&0\%&1.2\\
\hline
\multirow{4}*{ImageNet}&\multirow{4}*{ResNet50}&FGSM&95\%&95\%&0\%&0.08\\
~&~&BIM&99\%&{\bf 99\%}&0\%&0.11\\
~&~&C\&W&99\%&{94\%}&5.05\%&8.56\\
~&~&\tool&{\color{red} 96\%}&{\color{red} 96\%}&0\%&{\color{red} 37.2}\\
\hline
\multirow{4}*{ImageNet}&\multirow{4}*{InceptionV3}&FGSM&79\%&79\%&0\%&0.11\\
~&~&BIM&100\%&{\bf 100\%}&0\%&0.12\\
~&~&C\&W&100\%&68\%&32\%&1.41\\
~&~&\tool&{\color{red} 95\%}&{\color{red} 95\%}&0\%&{\color{red} 68.3}\\
\hline
\end{tabular}}
\end{table}

%\end{center}


\begin{table}[t]
  \centering
\caption{Results of white-box targeted attacks.}\label{tab:wt}
\resizebox{75mm}{!}{
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
{\bf Dataset}&{\bf DNN}&{\bf Method}&{\bf SR}&{\bf TSR}&{\bf GAP}&{\bf ATC}\\ \hline
\multirow{4}*{MNIST}&\multirow{4}*{LeNet-1}&FGSM&3\%&3\%&0\%&0\\
~&~&BIM&100\%&{\bf 100\%}&0\%&0.01\\
~&~&C\&W&100\%&70\%&0\%&24.5\\
~&~&\tool&100\%&{\bf 100\%}&0\%&3\\
\hline
\multirow{4}*{ImageNet}&\multirow{4}*{ResNet50}&FGSM&0\%&-&-&-\\
~&~&BIM&100\%&{\bf 100\%}&0\%&0.13\\
~&~&C\&W&99\%&62\%&37.37\%&19.85\\
~&~&\tool&{\color{red} \%}&{\color{red} \%}&0\%&{\color{red} }\\
\hline
\multirow{4}*{ImageNet}&\multirow{4}*{InceptionV3}&FGSM&0\%&-&-&-\\
~&~&BIM&99\%&{\bf 99\%}&0\%&0.19\\
~&~&C\&W&100\%&24\%&76\%&14.88\\
~&~&\tool&{\color{red} 92\%}&{\color{red} 92\%}&0\%&{\color{red} 309.2}\\
\hline
\end{tabular}}
\end{table}





\subsection{Comparison with Black-Box Methods}
%As mentioned above, the black-box methods are divided into two categories according to the need to train a new model. One is the substitution model that needs to train a new model, which is similar to the target model in structure and training set. After the new model is trained, apply the white-box method to generate adversarial examples, which may succeed on target model because of the migration aptitude. We chose the substitution model in the experiments of DeepXplore, which won the best paper in SOSP'17.

We compare \tool with several well-known
black-box methods: substitute model-based attacks,
ZOO~\cite{CZSYH17}, NES-PGD~\cite{IEAL18}, and GenAttack~\cite{ASCZHS19}.
In order to avoid the side-effect of the selected white-box methods when evaluating substitute model,
we use both the FGSM and C\&W methods respectively.
For ImageNet, we use ResNet50 as the substitute model for InceptionV3 and vice versa.
The substitute model for LeNet-1 is from the evaluation of ZOO~\cite{CZSYH17}.
Since our tool uses $\mathds{L}_\infty$ distance,
ZOO uses ${\bf L}_2$ distance.
We map the $\mathds{L}_\infty$ distances used in \tool to the corresponding approximated ${\bf L}_2$ distances in the experiments. In detail, we compute the ${\bf L}_2$ value for the worst case of $\mathds{L}_\infty$, that all the pixels are modified by $\mathds{L}_\infty$. It's worth to note that this is not a rigorous mapping, and the tool under ${\bf L}_2$, ZOO, would be easier to find an adversarial example, as this ${\bf L}_2$ limitation is less restricted.
Meanwhile, we remark that not all these tools provide related parameters for certain problems, in such cases,
we do not give their experimental results.


%The black-box methods we compared including substitution model,  alternative gradient based method (ZOO and NES-PGD), and decision-based method (DBA).
%In order to eliminate the impact of the selected white-box methods when evaluating substitution model, we use both the FGSM and C\&W methods respectively. For ImageNet, we use ResNet50 as the substitution model for InceptionV3 and vice versa. The substitution model for LeNet-1 is from the evaluation of ZOO~\cite{CZSYH17}.
%It is worth to note that, as our tool uses ${\bf L}_\infty$ distance, while DBA and ZOO use ${\bf L}_2$ distance. We map the ${\bf L}_\infty$ limitation used in \tool to the corresponding approximated ${\bf L}_2$ value in the experiments.  Meanwhile, some of the tools are dismissed in the table for certain problems because the corresponding tool has not given the related parameter for certain problem respectively.


The results of untargeted and targeted attacks are given in Table~\ref{tab:bu}  and Table~\ref{tab:bt} respectively.
We can see that our tool \tool significantly outperforms all the other tools in terms of TSR no matter targeted or untargeted attacks.
Substitute model based attacks can achieve at
most $38\%$ TSR under untargeted setting,
and $3\%$ TSR under targeted setting.
%
Compared with  ZOO~\cite{CZSYH17}, NES-PGD~\cite{IEAL18}, and GenAttack~\cite{ASCZHS19},% and DBA~\cite{RBB17},
our tool \tool can achieve similar or higher attack success rate in almost all the cases in terms of
SR.  However, all these methods suffer from the discretization problem, they usually have gaps between SR and TSR.
For instance, the attack success rate of ZOO is dramatically dropped from $73\%$ to $3\%$ on InceptionV3 in untargeted setting.


%
%
%In another category without a new model, we chose DBA, ZOO and NES-PGD for their excellent abilities. ZOO and NES-PGD generate the adversarial examples by calculating the simulated gradient, while DBA is a typical distance-oriented tool.

\begin{table}[t]
  \centering
\caption{Results of black-box untargeted attacks.}
\label{tab:bu}
\resizebox{85mm}{!}{
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
{\bf Dataset}&{\bf DNN}&{\bf Method}&{\bf SR}&{\bf TSR}&{\bf GAP}&{\bf ATC}\\
\hline
\multirow{5}*{MNIST}&\multirow{5}*{LeNet-1}&SModel+C\&W&2.5\%&2.5\%&0\%&28\\
~&~&SModel+FGSM&20\%&20\%&0\%&1\\
%~&~&DBA&99.5\%&84\%&15.58\%&11.89\\
~&~&ZOO&100\%&89.5\%&10.5\%&15.9\\
~&~&\tool&100\%&{\bf 100\%}&0\%&1.2\\
\hline
\multirow{4}*{ImageNet}&\multirow{4}*{ResNet50}&
SModel+C\&W&2\%&1\%&50\%&1.29\\
~&~&SModel+FGSM&24\%&24\%&0\%&0.12\\
%
%SModel+C\&W&0\%&-&-&-\\
%~&~&SModel+FGSM&0\%&-&-&-\\
%~&~&DBA&100\%&44\%&56\%&137.79\\
~&~&\tool&{\color{red} 96\%}&{\bf 96\%}&0\%&{\color{red} 37.2}\\
\hline
\multirow{7}*{ImageNet}&\multirow{7}*{InceptionV3}&
%SModel+C\&W&0\%&-&-&-\\
%~&~&SModel+FGSM&0\%&-&-&-\\
SModel+C\&W&6\%&6\%&0\%&24.32\\
~&~&SModel+FGSM&38\%&38\%&0\%&0.37\\
%~&~&Decision-Based&-&-&-&-\\
%~&~&DBA&100\%&34\%&66\%&254.2\\
~&~&ZOO&73\%&3\%&95.79\%&113\\
~&~&NES-PGD&100\%&77\%&23\%&24\\
~&~&{\color{red} GenAttack}&{\color{red} 100\%}&{\color{red} 83\%}&{\color{red} 17\%}&{\color{red} 18.7}\\
~&~&\tool&{\color{red} 95\%}&{\bf 95\%}&0\%&{\color{red} 68.3}\\
\hline
\end{tabular}}
\end{table}


\begin{table}[t]
  \centering
\caption{Results of black-box targeted attacks.}
\label{tab:bt}
\resizebox{85mm}{!}{
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
{\bf Dataset}&{\bf DNN}&{\bf Method}&{\bf SR}&{\bf TSR}&{\bf GAP}&{\bf ATC}\\
\hline
\multirow{5}*{MNIST}&\multirow{5}*{LeNet-1}&SModel+C\&W&1.5\%&1.5\%&0\%&22\\
~&~&SModel+FGSM&3\%&3\%&0\%&1\\
%~&~&DBA&95.5\%&79\%&17.28\%&12.17\\
~&~&ZOO&100\%&94.5\%&5.5\%&17.4\\
~&~&\tool&100\%&{\bf 100\%}&0\%&3\\
\hline
\multirow{4}*{ImageNet}&\multirow{4}*{ResNet50}&
SModel+C\&W&2\%&2\%&0\%&27.21\\
~&~&SModel+FGSM&-&-&-&-\\
%~&~&DBA&95\%&21\%&77.89\%&335\\
~&~&\tool&{\color{red} \%}&{\color{red} \%}&0\%&{\color{red} }\\
\hline
\multirow{7}*{ImageNet}&\multirow{7}*{InceptionV3}&
SModel+C\&W&1\%&1\%&0\%&41.66\\
~&~&SModel+FGSM&-&-&-&-\\
%~&~&DBA&87\%&25\%&71.3\%&544\\
~&~&ZOO&62\%&6\%&90.32\%&716.04\\
~&~&NES-PGD&100\%&47\%&53\%&56\\
~&~&{\color{red} GenAttack}&{\color{red} 100\%}&{\color{red} 72\%}&{\color{red} 28\%}&{\color{red} 52.2}\\
~&~&\tool&{\color{red} 92\%}&{\color{red} 92\%}&0\%&{\color{red} 309.2}\\
\hline
\end{tabular}}
\end{table}


%The results of our tool have been analyzed before, here mainly analyze and compare the others. Some research shows that substitution model does not work on large data sets such as ImageNet, which is consistent with our experimental results. As shown in Table2, substitution model performs poorly no matter which white-box method is applied. The ASR of all the others can not reach 100\% even 50\% in target attack because of that they all perform in float-point domain especially ZOO and Decision-based. Thus the TSR of our tool is much higher than the others.

%\subsection{Analysis of ASR}
%Most methods generate adversarial examples with an iterative process, with only a few changes in float-point domain in each iteration. There are two advantages through the above process, one is that the altered image is as close as original image while another is that the process of generation is more stable and more likely to succeed. However, the consequence is that some methods actually find some examples in float-point domain, which should exist in real world and need to be transformed into integer domain in computer vision with loss of significance. Our method does not need to consider the distance between altered image and original image because of that the distance is fixed before execution, thus our method can sample from integer domain to keep 100\% ASR.

\subsection {Efficiency Analysis}
\noindent\textbf{Time cost.} From Table~\ref{tab:wu} to Table~\ref{tab:bt},
we can see that the time cost of \tool varies in different cases.
On small models and images from MNIST, the average time cost of \tool is very small, around 1--3 seconds;
while on larger models and images from ImageNet, the time cost is increased to at most $375$ seconds.
The reason is that we change the values of two coordinates for each sample on MNIST images,
while change the values of 600 coordinates for each sample on ImageNet images.
Thus, it spends more time to handle these modifications, and the time cost is significantly increased on ImageNet images.
We remark that under black-box scenarios,
the time cost of our tool \tool is on the same level as other non-substitute model-based tools in most cases,
moreover, the time cost of \tool is the average time cost per integer
adversarial example instead of real
adversarial example.


%we only make the perturbation on at most 2 coordinates of each sample, while for ImageNet, we change the threshold to 600 coordinates of a sample. Therefore, we need to spend more time to handle these modifications, and the time usage is significantly increased and higher than the other tools in large cases, i.e. ImageNet.

%On the other hand, if we focus on the black-box attack, we can see the time usage of our method is on the same level as other non-substitution model-based tools basically in most of the problems.


\begin{table}[t]
  \centering
\caption{Comparison with NES-PGD, Bandit and GenAttack with average query times of success cases.}\label{tab:query}
\resizebox{85mm}{!}{
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
&&&\multicolumn{2}{|c|}{Untargeted attack}&\multicolumn{2}{|c|}{Targeted attack}\\
\cline{4-7}
\raisebox{1ex}{Dataset}&\raisebox{1ex}{DNN}&\raisebox{1ex}{Method}&TSR&AVQ&TSR&AVQ\\\hline
\multirow{5}*{ImageNet}&\multirow{5}*{InceptionV3}&NES-PGD&77\%&4741&47\%&13421\\
~&~&{Bandit}&running&3255&-&-\\
~&~&{\color{red} GenAttack}&83\%&{\color{red} 2964}&72\%&{\color{red} 9177}\\
~&~&Our tool&83\%&2170&72\%&9997\\
~&~&Our tool&95\%&3831&92\%&20131\\
\hline
\end{tabular}}
\end{table}

\medskip
\noindent\textbf{Comparing query times with NES-PGD~\cite{IEAL18}, Bandit~\cite{IEM2018PriorCB} and GenAttack~\cite{ASCZHS19}.}
In many black-box scenarios, there may exist a limitation of query times to avoid detection.
Therefore, in the context of black-box attacks, query efficiency should be considered.
%
We compare the number of queries of \tool against two of the most query-efficient methods:
NES-PGD~\cite{IEAL18} and Bandit~\cite{IEM2018PriorCB}, where
NES-PGD is a natural evolutionary-based tool and Bandit is an optimized version of NES-PGD by using bandit optimization.
NES-PGD and Bandit are black-box attack tools which focus on query-limited scenarios.
%%
We use InceptionV3 as the targeted classifier and
conduct both untargeted and targeted attacks using NES-PGD, Bandit
and our tool \tool. [The parameter setting of Bandit for targeted attack is not given therein, therefore we only conduct untargeted attacks for Bandit.]
The average query times per successful attack used by each tool is given in Table~\ref{tab:query}.
We can see that \tool outperforms the other two tools in terms for query times.
It is worth mentioning that the query times of our tool is computed on integer adversarial examples,
while it is computed on real adversarial examples for NES-PGD and Bandit.


%% This part can combine with Efficiency Analysis part.
%\begin{table}[t]
%\centering
%\small
%\caption{Results of \tool on different $\mathds{L}_\infty$ distances}\label{tab:zhaozheavg}
%%\resizebox{65mm}{!}{
%\begin{tabular}{|c|c|c|c|}
%\hline
% $\epsilon$ & {\bf Max times} & {\bf Mean of times} & {\bf ATC}\\
%\hline
%% 16 & 85933 & 4691 & 4.41 \\
%32 & 85933 & 4691 & 4.41 \\
%64 & 3902 & 682 & 1.2 \\
%76 & 2213 & 466 & 0.61 \\
%\hline
%\end{tabular}%}
%\end{table}
%
%\medskip
%% add by Zhaozhe
%\noindent\textbf{Performance of \tool on different $\mathds{L}_\infty$ distances.}
%To understand the performance of our tool \tool on different $\mathds{L}_\infty$ distances,
%we run \tool with $\epsilon=32,64,76$ on the 200 MNIST images with untargeted attacks.
%The results are shown in Table~\ref{tab:zhaozheavg}.
%It is easy to see that the larger of the $\mathds{L}_\infty$ distance, the more
%efficient of \tool.
%When $\epsilon=64,76$, \tool only take several hundreds of queries and nearly 1 second
%to craft an integer adversarial example without computing gradient.
%On MNIST dataset, DFA is faster than many white-box attacks and as our best known,
%DFA is one of the fastest black box methods with such a high ASR.


% shows DFA efficiency is affected by the problem`s difficulty and the size of search space,
%the efficiency of DFA can be significantly improved when the problem`s solution density of the search space is higher.
%When we set $\mathds{L}_\infty$ to $64/255$ or $76/255$,
%DFA only need 1 second and several hundreds queries to find a solution without
%calculate the gradient and iterative optimization according to the direction of gradient.


%\medskip
%% add by Zhaozhe
%\noindent\textbf{Uniform Distribution.}
%Unlike FGSM that can only craft one adversarial examples for each input image under same step size,
%\tool is able to craft different adversarial examples for each input image under same parameters, due to its inherent random characteristic.
%For each MNIST image, we use \tool to craft five adversarial examples consecutively with same parameters as shown in Table~\ref{tab:set}.
%The $\mathds{L}_2$ distances between these examples and the original image are shown in Table~\ref{tab:zhaozheuniform}.
%We can observe that the distances are very uniform.
%This demonstrates that \tool  quickly craft multiple different adversarial examples for a given image.
%
%\begin{table}[t]
%\centering
%\small
%\caption{$\mathds{L}_2$ distance on different examples}\label{tab:zhaozheuniform}
%%\resizebox{65mm}{!}{
%\begin{tabular}{|c|c|c|c|c|c|c|c|}
%\hline
%& {\bf RAW} & {\bf 1}    & {\bf 2}    &{\bf 3}    & {\bf 4}    &{\bf 5}   & {\bf Query Times}     \\
%\hline
%{\bf RAW} & 0.00 & 1.20 & 1.23 & 1.21 & 1.21 & 1.24        & -    \\
%\hline
%{\bf 1}   & 1.20 & 0.00 & 1.33 & 1.36 & 1.36 & 1.33        & 329 \\
%\hline
%{\bf 2}   & 1.23 & 1.33 & 0.00 & 1.31 & 1.37 & 1.40        & 226 \\
%\hline
%{\bf 3}   & 1.21 & 1.36 & 1.31 & 0.00 & 1.38 & 1.36        & 398 \\
%\hline
%{\bf 4}   & 1.21 & 1.36 & 1.37 & 1.38 & 0.00 & 1.34        & 422 \\
%\hline
%{\bf 5}   & 1.24 & 1.33 & 1.40 & 1.36 & 1.34 & 0.00        & 327 \\
%\hline
%\end{tabular}
%\end{table}

% uses the smallest number of query times compared with these two works focusing on query-limited problems. The reason is that, after each query, our method makes a deep investigation of the queried samples to refine the search space accordingly. Therefore, our tool can achieve a much better query time and this also explains why the total time usage of our tool is larger compared with other tools.


%In many black-box scenarios, it is not rare to see a limitation of query times to avoid detection. Therefore, we also compare the query time of our tools with two black-box tools which focus on query-limited scenarios. These %tools are NES-PGD and Bandit~\cite{IEM2018PriorCB}, which coming from the same group of authors. Bandit is an optimized version of NES-PGD that Bandit uses bandit optimization, while NES-PGD is natural evolutionary-based.

%We run these two tools and also our \tool on the InceptionV3 model in the untargeted attack mode. The average query times used by each tool in the successful attack cases is reported in Table~\ref{tab:query}\footnote{The parameter setting of Bandit on targeted attack is not given, therefore we only run Bandit in the untargeted mode.}. We can see that our tool uses the smallest number of query times compared with these two works focusing on query-limited problems. The reason is that, after each query, our method makes a deep investigation of the queried samples to refine the search space accordingly. Therefore, our tool can achieve a much better query time and this also explains why the total time usage of our tool is larger compared with other tools.


\subsection{Attack Classifiers with Defense}
To show the effectiveness of our approach,
we first use our tool to attack the HGD defense~\cite{LLDPH018}, which won the first place of
NIPS 2017 competition on defense against adversarial attacks.


In this experiment, we conduct untargeted attacks on this model
using the same 100 images from ImageNet as previously.
The $\mathds{L}_\infty$ distance $\epsilon$ is $32$ according to the competition's setting.
The coordinate threshold is set to $200$.
Our tool achieves $72\%$ attack success rate with  30 minute time limitation for each attack.
The attack success rate significantly increases to $95\%$ with 200 minutes time limitation.
This demonstrates that \tool is able to handle difficult problems with enough computation resource.

%
%
%Firstly, we attack the model by time limitation set to $30$ minutes and happily achieve the success rate of $72\%$.
% We take a further investigation and find out that all the unsuccessful attacks are stopped due to the time limitation, and the average iteration they achieved is $1077$ rounds.
% As defense system is much more difficult to attack than the normal network, we make another set of experiments, that we dismiss the time limitation and let \tool run until the iteration limitation is reached. Then, the success rate is significantly increased to $95\%$?For the new successfully attacked $23$ images, the average iteration round is $2482$. This also confirms our argument that we can use our method to handle difficult problems with enough computation resource.



%
%As our tool is black-box based, we have no such limitation. Therefore, we also try to use our tool to attack the HGD defense~\cite{LLDPH018}, which won the first place of
%NIPS 2017 competition on defense against adversarial attacks.
%
%
%Recently, there are many works discussing how to increase the robustness of networks by different methods like gradient obfuscation, adversarial detection and so on. Most of the white-box methods have difficulties in attacking such defense methods as gradient information is not easy to fetch under such techniques. As our tool is black-box based, we have no such limitation. Therefore, we also try to use our tool to attack the HGD defense~\cite{LLDPH018}, which won the first place of
%NIPS 2017 competition on defense against adversarial attacks.
%
%In the experiment, we attack this model in the untargeted mode, using the same 100 images from ImageNet as used in the previous experiments. The $\mathds{L}_\infty$ distance $\epsilon$ is set to $32$ according to the competition's setting. The coordinate threshold is set to $200$.
%
%Firstly, we attack the model by time limitation set to $30$ minutes and happily achieve the success rate of $72\%$.  We take a further investigation and find out that all the unsuccessful attacks are stopped due to the time limitation, and the average iteration they achieved is $1077$ rounds. As defense system is much more difficult to attack than the normal network, we make another set of experiments, that we dismiss the time limitation and let \tool run until the iteration limitation is reached. Then, the success rate is significantly increased to $95\%$?For the new successfully attacked $23$ images, the average iteration round is $2482$. This also confirms our argument that we can use our method to handle difficult problems with enough computation resource.
%
%
%



%As this problem is much harder than other problems, we give no time limitation in the experiment.  And we are happy to see that we achieve $xx\%$ success rate in the experiment.

On MNIST Adversarial Examples Challenge~\cite{mnistchallenge19},
another widely recognized attack problem, we use the same 200 MNIST images as previously.
Our tool \tool achieves $10.5\%$ attack success rate, the same as the current best white-box attack ``interval attacks'', which is publicly reported on the webpage of the challenge.
Indeed, the images crafted by both methods are exactly the same, and the time costs of both tools are also similar.
%This result greatly strengths our belief that our method can be used to handle difficult problems with satisfactory success rate.


%\begin{table}[htbp]
%  \centering
%\caption{Defense Attack}\label{tab:def}
%\resizebox{85mm}{!}{
%\begin{tabular}{|c|c|c|c|}
%\hline
%Dataset&Defense Method&Success Rate&Average Time/min\\
%\hline
%ImageNet&Guided-Denoise&62\%&14\\
%\hline
%\end{tabular}}
%\end{table}
%
%%\textbf{Table 6}~~Effect on network with defense.\\
%\end{center}
%\subsection{Parameter Discussion}
%Last but not least, we make a discussion about how our method will be affected by the parameters. The parameters used in the experiment are summarized in Table~\ref{tab:set}. We have not made a complete grid search of the best parameter setting for each problem. Instead, we give a few isolated sets of parameters intuitively for different problems respectively.
%
%
%Among the parameters listed in the table, obviously, the larger $\mathds{L}_\infty$ distance is, the simpler the problem will be. The larger the time limitation is, the higher the success rate will be. Meanwhile, if we give our algorithm more computation resource, i,e, iteration rounds and larger coordinate threshold, the algorithm can be used to handle difficult problems as shown in the previous analysis of time usage and defense system. Due to the space limitation, here we mainly focus on the discussion about the effect of the sample size in each round.
%
%We conduct untargeted attack on the InceptionV3 network. The sample size $s$ is set to $3$,$5$, $7$, and $10$ respectively. The data is reported in Table~\ref{tab:eff}. From the data, we can clearly see that with the increase of the sample size, the success rate is increased from $93\%$ to $97\%$. Meanwhile, the time usage and query times are increased as well. This is consistent with our understanding that with more samples in each iteration, \tool needs to spend more time in the evaluation of each sample and also perturbation generation. Meanwhile, as \tool can achieve more information from the added samples, the success rate is increased as a result.
%
%\begin{table}[t]
%  \centering
%\caption{Performance of \tool Under Different Sample Size}\label{tab:eff}
%%\resizebox{65mm}{!}{
%\begin{tabular}{|c|c|c|c|}
%\hline
%Sample size&TSR&ATC&Query times\\
%\hline
%3&93\%&106.8&2660\\
%5&96\%&137.4&3739\\
%7&95\%&134.4&3854\\
%10&97\%&150.6&4327\\
%\hline
%\end{tabular}%}
%\end{table}

%
%\section{Related Work}
%\label{sec:rel}


==> experiments2.tex <==
\section{Self-comparison Experiments}
\label{sec:expr2}
In this experiment, we compare the performance of our tool with different value of parameters including $\mathds{L}_\infty$ distance, sample size and coordinate threshold. The results are shown in Table~\ref{tab:scmp}, Table~\ref{tab:scs} and Table~\ref{tab:scub}.

All the self-comparison experiments from Table~\ref{tab:scmp} to Table~\ref{tab:scub} are targeted attack on the ImageNet dataset with InceptionV3 as the targeted DNN classifier. We only modify one parameter for each experiment, keeping the other parameters unchanged. Specifically, we set coordinate threshold to 600, sample size to 10 and $\mathds{L}_\infty$ distance to 10 when they are unchanged, which is consistent with previous settings.
\subsection{Self-comparison Experiments about $\mathds{L}_\infty$ distance}
$\mathds{L}_\infty$ distance represents the distance between adversary example and original image. The higher $\mathds{L}_\infty$ distance, the larger search space and the simpler problem. In this experiment, we set $\mathds{L}_\infty$ distance to 15, 10 and 5 respectively. When $\mathds{L}_\infty$ distance is very small, as the $\mathds{L}_\infty$ distance decreases, the difficulty of the problem has increased significantly. As expected in Table~\ref{tab:scmp}, the SR decreases, the query times and ATC increase with the decreasing of $\mathds{L}_\infty$ distance.

\begin{table}[t]
  \centering
\caption{Results of the change of $\mathds{L}_\infty$ distance}
\label{tab:scmp}
\resizebox{85mm}{!}{
\begin{tabular}{|c|c|c|c|c|c|}\hline
Coordinate Threshold&Sample size&$\mathds{L}_\infty$ distance&SR&query times&ATC\\
\hline
\multirow{3}*{600}&\multirow{3}*{10}&15&83\%&10377&370\\
~&~&10&72\%&11364&375\\
~&~&5&56\%&14259&509\\
\hline
\end{tabular}}
\end{table}

\subsection{Self-comparison Experiments about Sample Size}
Sample size represents the sampling breadth of each iteration of the DFA, theoretically, the larger sample size, the better sampling. In this experiment, we set sample size to 5, 10, 15 and 20 respectively. However, as shown in Table~\ref{tab:scs}, unexpectedly, when the sample size is 15, the SR is not significantly higher than that sample size is 10. Even more, when sample size is 20, the SR is declining. This is because that the larger sample size, the smaller iteration threshold in same time out. Therefore, the decrease of iteration threshold results in that the optimization process still does not reach convergence when the time resources run out. In order to compare the impact of sample size objectively, we should unify the iteration threshold instead of time out.

\begin{table}[t]
  \centering
\caption{Results of the change of Sample size}
\label{tab:scs}
\resizebox{85mm}{!}{
\begin{tabular}{|c|c|c|c|c|c|}\hline
Coordinate Threshold&$\mathds{L}_\infty$ distance&Sample size&SR&query times&ATC\\
\hline
\multirow{5}*{600}&\multirow{5}*{10}&3&66\%&6624&281\\
~&~&5&73\%&10189&390\\
~&~&10&72\%&11364&375\\
~&~&15&73\%&12146&409\\
~&~&20&69\%&9900&368\\
\hline
\end{tabular}}
\end{table}

\subsection{Self-comparison Experiments about Coordinate Threshold}
Coordinate threshold indicates the degree of change in each iteration, which is similar to the step size in other methods. The larger coordinate threshold, the larger change in each iteration, the smaller the search granularity and the faster the convergence rate. In this experiment, we set coordinate threshold to 200, 400, 600, 800 and 1000 respectively. As shown in Table~\ref{tab:scub}, as expected, the smaller coordinate threshold, the higher SR and the higher ATC except when coordinate threshold is 800. This is because that fast convergence only means finding a local optimum quickly, which may not be a successful case. So the ATC when coordinate threshold is 1000 is higher than that is 800.


\begin{table}[t]
  \centering
\caption{Results of the change of Coordinate Threshold}
\label{tab:scub}
\resizebox{85mm}{!}{
\begin{tabular}{|c|c|c|c|c|c|}\hline
Sample size&$\mathds{L}_\infty$ distance&Coordinate Threshold&SR&query times&ATC\\
\hline
\multirow{5}*{10}&\multirow{5}*{10}&200&88\%&14308&489\\
~&~&400&80\%&12582&438\\
~&~&600&72\%&11364&375\\
~&~&800&68\%&9451&336\\
~&~&1000&68\%&10053&360\\
\hline
\end{tabular}}
\end{table}

